Rigorous Deductive Argumentation for Socially Relevant Issues

The most important problems for society are describable only in vague terms, dependent on subjective positions, and missing highly relevant data. This thesis is intended to revive and further develop the view that giving non-trivial, rigorous deductive arguments concerning such problems -without eliminating the complications of vagueness, subjectivity, and uncertainty- is, though very difficult, not problematic in principle, does not require the invention of new logics -classical first-order logic will do- and is something that more mathematically-inclined people should be pursuing. The framework of interpreted formal proofs is presented for formalizing and criticizing rigorous deductive arguments about vague, subjective, and uncertain issues, and its adequacy is supported largely by a number of major examples. This thesis also documents progress towards a web system for collaboratively authoring and criticizing such arguments, which is the ultimate goal of this project.

==> RelatedWork.tex <==
%!TEX root = ../thesis.tex

\subsection{\Blue{Informal Logic}}
Start with stuff from research/thesis proposal.

\subsection{\Blue{Abstract Argumentation Systems}}
Start with stuff from research/thesis proposal.

\subsection{The Logical Positivists}
The logical positivists worked to varying degrees to expand the applications of formal logic to areas outside traditional mathematics, especially science. According to the most vocal of modern commentators, they were largely unsuccessful. It seems that the creation of a \TODO[\LDS] (see Section \ref{s:LeibnitzianDialogDystems}) would have been considered very worthwhile among the logical positivists, and unlike Leibniz, they did have modern formal logic at their disposal. Given that, I attribute their lack of progress to two main factors:
\begin{PPE}
\item Preoccupation with constructing elegant, widely-applicable theories. 
A premise of my approach is that an informal yes/no question must be fixed before formalization begins. Hence, the development of general theories about subjective and vague matters is explicitly not a goal; only making progress on the question matters. Of course, abstracting out common axiomatizations for reuse is still a good idea, but as with writing software libraries, it should not be done preemptively.
\item Working with examples outside of the problem domain I outlined in Section \ref{s:problemdomain}. Because there is less promise of discovering mathematically interesting material in the formal investigation of a question about a vague and subjective issue, the motivation for the very difficult work involved in rigorous reasoning must come entirely from elsewhere, namely from the question itself; we must be convinced that there is no easier way to make progress on the question, and that making progress on the question is indeed worth the work. Leibniz knew the danger of being insufficiently conscious of this point; speculating about why the project he envisioned had not been taken up by others earlier, like Descartes, he wrote:
\begin{aquote}{Gottfried Leibniz, 1679, \textit{On the General Characteristic} \cite{leibniz1976}}
{\it 
The true reason for this straying from the portal of knowledge is, I believe, that principles usually seem dry and not very attractive and are therefore dismissed with a mere taste.}
\end{aquote}
Also, the stigma in mathematics and science against working toward progress on value-laden issues has grown over time. Doing so gets one's work labeled as philosophy. The stigma is not surprising, given what has passed as good work in contemporary philosophy, but on the other hand, it is a clear fallacy of association to condemn a subject of study on account of the people who have managed, so far, to get paid to work on it. %It is related to the fear of being labeled a philosopher, which on one is u
\end{PPE}

%\subsection{\Blue{Deontic Logic}}

%\subsection{\Blue{Logic for Law}} \label{s:LogicForLaw}

\subsection{\Blue{Theories for Formalizing Defeasible Legal Arguments}}

\subsection{\Blue{Logic-related Computer Tool Support for Lawyers}}
Quote Lovevinger page 511

\subsection{\Blue{Logic to Make Law More Just}}

FYI: moved Lovevinger quote to intro.

\subsection{\Blue{Natural language semantics, Montague grammar, constructed languages}} \label{s:naturallanguage}



